An Actor-Critic-Attention Mechanism for Deep Reinforcement Learning in Multi-view Environments

In reinforcement learning algorithms, leveraging multiple views of the environment can improve the learning of complicated policies. In multi-view environments, due to the fact that the views may frequently suffer from partial observability, their level of importance are often different. In this paper, we propose a deep reinforcement learning method and an attention mechanism in a multi-view environment. Each view can provide various representative information about the environment. Through our attention mechanism, our method generates a single feature representation of environment given its multiple views. It learns a policy to dynamically attend to each view based on its importance in the decision-making process. Through experiments, we show that our method outperforms its state-of-the-art baselines on TORCS racing car simulator and three other complex 3D environments with obstacles. We also provide experimental results to evaluate the performance of our method on noisy conditions and partial observation settings.

==> del <==
@book{sutton1998reinforcement,
 title={Reinforcement learning: An introduction},
 author={Sutton, Richard S and Barto, Andrew G},
 volume={1},
 number={1},
 year={1998},
 publisher={MIT press Cambridge}
}
@inproceedings{ren2017deep,
  title={Deep reinforcement learning-based image captioning with embedding reward},
  author={Ren, Zhou and Wang, Xiaoyu and Zhang, Ning and Lv, Xutao and Li, Li-Jia},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={290--298},
  year={2017}
}
@inproceedings{kong2017collaborative,
  title={Collaborative deep reinforcement learning for joint object search},
  author={Kong, Xiangyu and Xin, Bo and Wang, Yizhou and Hua, Gang},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1695--1704},
  year={2017}
}
@article{el2017deep,
 title={Deep Reinforcement Learning framework for Autonomous Driving},
 author={El Sallab, Ahmad and Abdou, Mohammed and Perot, Etienne and Yogamani, Senthil},
 journal={Autonomous Vehicles and Machines, Electronic Imaging},
 year={2017}
}
@article{bojarski2016end,
 title={End to end learning for self-driving cars},
 author={Bojarski, Mariusz and Del Testa, Davide and Dworakowski, Daniel and Firner, Bernhard and Flepp, Beat and Goyal, Prasoon and Jackel, Lawrence D and Monfort, Mathew and Muller, Urs and Zhang, Jiakai and others},
 journal={arXiv preprint arXiv:1604.07316},
 year={2016}
}
@article{fridman2018deeptraffic,
 title={DeepTraffic: Driving Fast through Dense Traffic with Deep Reinforcement Learning},
 author={Fridman, Lex and Jenik, Benedikt and Terwilliger, Jack},
 journal={arXiv preprint arXiv:1801.02805},
 year={2018}
}
@article{shalev2016safe,
 title={Safe, multi-agent, reinforcement learning for autonomous driving},
 author={Shalev-Shwartz, Shai and Shammah, Shaked and Shashua, Amnon},
 journal={arXiv preprint arXiv:1610.03295},
 year={2016}
}
@inproceedings{koutnik2013evolving,
 title={Evolving large-scale neural networks for vision-based reinforcement learning},
 author={Koutn{\'\i}k, Jan and Cuccu, Giuseppe and Schmidhuber, J{\"u}rgen and Gomez, Faustino},
 booktitle={GECCO},
 pages={1061--1068},
 year={2013},
 organization={ACM}
}
@inproceedings{schulman2015trust,
 title={Trust region policy optimization},
 author={Schulman, John and Levine, Sergey and Abbeel, Pieter and Jordan, Michael and Moritz, Philipp},
 booktitle={ICML},
 pages={1889--1897},
 year={2015}
}
@article{you2017virtual,
 title={Virtual to Real Reinforcement Learning for Autonomous Driving},
 author={You, Yurong and Pan, Xinlei and Wang, Ziyan and Lu, Cewu},
 journal={arXiv preprint arXiv:1704.03952},
 year={2017}
}
@article{kober2013reinforcement,
 title={Reinforcement learning in robotics: A survey},
 author={Kober, Jens and Bagnell, J Andrew and Peters, Jan},
 journal={IJRR},
 volume={32},
 number={11},
 pages={1238--1274},
 year={2013},
 publisher={SAGE Publications Sage UK: London, England}
}
@article{lecun2015deep,
 title={Deep learning},
 author={LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
 journal={Nature},
 volume={521},
 number={7553},
 pages={436--444},
 year={2015},
 publisher={Nature Research}
}
@inproceedings{pomerleau1989alvinn,
 title={Alvinn: An autonomous land vehicle in a neural network},
 author={Pomerleau, Dean A},
 booktitle={NIPS},
 pages={305--313},
 year={1989}
}
@inproceedings{koutnik2013evolving,
 title={Evolving large-scale neural networks for vision-based reinforcement learning},
 author={Koutn{\'\i}k, Jan and Cuccu, Giuseppe and Schmidhuber, J{\"u}rgen and Gomez, Faustino},
 booktitle={GECCO},
 pages={1061--1068},
 year={2013},
 organization={ACM}
}
@inproceedings{koutnik2014evolving,
 title={Evolving deep unsupervised convolutional networks for vision-based reinforcement learning},
 author={Koutn{\'\i}k, Jan and Schmidhuber, J{\"u}rgen and Gomez, Faustino},
 booktitle={GECCO},
 pages={541--548},
 year={2014},
 organization={ACM}
}
@inproceedings{schaul2015prioritized,
 title={Prioritized experience replay},
 author={Schaul, Tom and Quan, John and Antonoglou, Ioannis and Silver, David},
 booktitle={ICLR},
 year={2016}
}
@inproceedings{van2016deep,
 title={Deep Reinforcement Learning with Double Q-Learning},
 author={Van Hasselt, Hado and Guez, Arthur and Silver, David},
 booktitle={AAAI},
 pages={2094--2100},
 year={2016}
}
@inproceedings{wang2015dueling,
 title={Dueling network architectures for deep reinforcement learning},
 author={Wang, Ziyu and Schaul, Tom and Hessel, Matteo and Van Hasselt, Hado and Lanctot, Marc and De Freitas, Nando},
 booktitle={ICML},
 year={2016}
}
@article{bellemare2013arcade,
 title={The Arcade Learning Environment: An evaluation platform for general agents},
 author={Bellemare, Marc G and Naddaf, Yavar and Veness, Joel and Bowling, Michael},
 journal={JAIR},
 volume={47},
 pages={253--279},
 year={2013}
}
@inproceedings{mnih2013playing,
 title={Playing atari with deep reinforcement learning},
 author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Graves, Alex and Antonoglou, Ioannis and Wierstra, Daan and Riedmiller, Martin},
 booktitle={NIPS Workshop on Deep Learning},
 year={2013}
}
@inproceedings{pomerleau1992neural,
 title={Neural network perception for mobile robot guidance},
 author={Pomerleau, Dean A},
 booktitle={IV Symposium},
 year={1992}
}
@inproceedings{chen2015deepdriving,
 title={Deepdriving: Learning affordance for direct perception in autonomous driving},
 author={Chen, Chenyi and Seff, Ari and Kornhauser, Alain and Xiao, Jianxiong},
 booktitle={ICCV},
 pages={2722--2730},
 year={2015}
}
@article{liu2017learning,
  title={Learning End-to-end Multimodal Sensor Policies for Autonomous Navigation},
  author={Liu, Guan-Horng and Siravuru, Avinash and Prabhakar, Sai and Veloso, Manuela and Kantor, George},
  journal={arXiv preprint arXiv:1705.10422},
  year={2017}
}
@inproceedings{ciosek2017offer,
 title={OFFER: Off-Environment Reinforcement Learning},
 author={Ciosek, Kamil Andrzej and Whiteson, Shimon},
 booktitle={AAAI},
 pages={1819--1825},
 year={2017}
}
@inproceedings{zhang2017query,
 title={Query-Efficient Imitation Learning for End-to-End Simulated Driving},
 author={Zhang, Jiakai and Cho, Kyunghyun},
 booktitle={AAAI},
 pages={2891--2897},
 year={2017}
}
@inproceedings{wolf2017learning,
 title={Learning how to drive in a real world simulation with deep Q-Networks},
 author={Wolf, Peter and Hubschneider, Christian and Weber, Michael and Bauer, Andr{\'e} and H{\"a}rtl, Jonathan and D{\"u}rr, Fabian and Z{\"o}llner, J Marius},
 booktitle={IV Symposium},
 pages={244--250},
 year={2017},
 organization={IEEE}
}
@article{bojarski2017explaining,
 title={Explaining How a Deep Neural Network Trained with End-to-End Learning Steers a Car},
 author={Bojarski, Mariusz and Yeres, Philip and Choromanska, Anna and Choromanski, Krzysztof and Firner, Bernhard and Jackel, Lawrence and Muller, Urs},
 journal={arXiv preprint arXiv:1704.07911},
 year={2017}
}
@article{kim2017interpretable,
 title={Interpretable Learning for Self-Driving Cars by Visualizing Causal Attention},
 author={Kim, Jinkyu and Canny, John},
 journal={ICCV},
 year={2017}
}
@article{chi2017deep,
  title={Deep Steering: Learning End-to-End Driving Model from Spatial and Temporal Visual Cues},
  author={Chi, Lu and Mu, Yadong},
  journal={arXiv preprint arXiv:1708.03798},
  year={2017}
}
@article{mirowski2016learning,
  title={Learning to navigate in complex environments},
  author={Mirowski, Piotr and Pascanu, Razvan and Viola, Fabio and Soyer, Hubert and Ballard, Andrew J and Banino, Andrea and Denil, Misha and Goroshin, Ross and Sifre, Laurent and Kavukcuoglu, Koray and others},
  journal={arXiv preprint arXiv:1611.03673},
  year={2016}
}
